Globular cluster systems and galaxy formation

Globular clusters are compact, gravitationally bound systems of up to a million stars. The GCs in the Milky Way contain some of the oldest stars known, and provide important clues to the early formation and continuing evolution of our Galaxy. More generally, GCs are associated with galaxies of all types and masses, from low-mass dwarf galaxies to the most massive early-type galaxies which lie in the centres of massive galaxy clusters. GC systems show several properties which connect tightly with properties of their host galaxies. For example, the total mass of GCs in a system scales linearly with the dark matter halo mass of its host galaxy. Numerical simulations are at the point of being able to resolve globular cluster formation within a cosmological framework. Therefore, GCs link a range of scales, from the physics of star formation in turbulent gas clouds, to the large-scale properties of galaxies and their dark matter. In this Chapter we review some of the basic observational approaches for GC systems, some of their key observational properties, and describe how GCs provide important clues to the formation of their parent galaxies.

==> references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 

% Journal article


\bibitem{Alabi2017} Alabi, A.~B., Forbes, D.~A., Romanowsky, A.~J., et al.\ 2017, MNRAS, 468, 3949 
\bibitem{2011MNRAS.417.1823A} Alves-Brito, A., Hau, G.~K.~T., Forbes, D.~A., et al.\ 2011, MNRAS, 417, 1823
\bibitem{2014ApJ...791...80A} Arnold, J.~A., Romanowsky, A.~J., Brodie, J.~P., et al.\ 2014, ApJ, 791, 80
\bibitem{1992ApJ...384...50A} Ashman, K.~M., \& Zepf, S.~E.\ 1992, ApJ, 384, 50 
\bibitem{2001PhR...349..125B} Barkana, R., \& Loeb, A.\ 2001, Physics Reports, 349, 125 
\bibitem{}Bastian N., Lardo C., 2018, ARA\&A, 56, 83
\bibitem{2019MNRAS.487.1986B} Beasley, M.~A., Leaman, R., Gallart, C., et al.\ 2019, MNRAS, 487, 1986
\bibitem{2018Natur.555..483B} Beasley, M.~A., Trujillo, I., Leaman, R., \& Montes, M.\ 2018, Nature, 555, 483 
\bibitem{2016ApJ...819L..20B} Beasley, M.~A., Romanowsky, A.~J., Pota, V., et al.\ 2016, ApJL, 819, L20
\bibitem{2008MNRAS.386.1443B} Beasley, M.~A., Bridges, T., Peng, E., et al.\ 2008, MNRAS, 386, 1443
\bibitem{2002MNRAS.333..383B} Beasley, M.~A., Baugh, C.~M., Forbes, D.~A., Sharples, R.~M., \& Frenk, C.~S.\ 2002, MNRAS, 333, 383 
\bibitem{2003MNRAS.346L..11B} Bekki, K., \& Freeman, K.~C.\ 2003, MNRAS, 346, L11
\bibitem{2017MNRAS.467.2446B} Binney, J., \& Wong, L.~K.\ 2017, MNRAS, 467, 2446
\bibitem{}Bland-Hawthorn, J., \& Gerhard, O.\ 2016, ARA\&A 54, 529
\bibitem{2017arXiv171102090B} Bouwens, R.~J., Illingworth, G.~D., Oesch, P.~A., et al.\ 2017, arXiv:1711.02090 
\bibitem{2018MNRAS.479..332B} Boylan-Kolchin, M.\ 2018, MNRAS, 479, 332 
\bibitem{2014MNRAS.439.2420B} Blom, C., Forbes, D.~A., Foster, C., Romanowsky, A.~J., \& Brodie, J.~P.\ 2014, MNRAS, 439, 2420 
\bibitem{}Blom, C., Forbes, D.~A., Brodie, J.~P., et al.\ 2012, MNRAS, 426, 1959 
\bibitem{}Brodie, J.~P., \& Strader, J. 2006, ARA\&A, 44, 193
\bibitem{2003MNRAS.344.1000B} Bruzual, G., \& Charlot, S.\ 2003, MNRAS, 344, 1000
\bibitem{2009MNRAS.394..929C} Cacciato, M., van den Bosch, F.~C., More, S., et al.\ 2009,MNRAS, 394, 929
\bibitem{2011AJ....141...61C} Caldwell, N., Schiavon, R., Morrison, H., et al.\ 2011, AJ, 141, 61
\bibitem{}Cappellari, M.\ 2016, ARA\&A, 54, 597
\bibitem{2010A&A...520A..95C} Carretta, E., Bragaglia, A., Gratton, R.~G., et al.\ 2010, AAP, 520, A95
\bibitem{2007AJ....134..391C} Cenarro, A.~J., Beasley, M.~A., Strader, J., et al.\ 2007,AJ, 134, 391
\bibitem{1996MNRAS.283..683C} Chaboyer, B., Demarque, P., Kernan, P.~J., et al.\ 1996, MNRAS, 283, 683
\bibitem{2012MNRAS.427.2349C} Chies-Santos, A.~L., Larsen, S.~S., \& Kissler-Patig, M.\ 2012, MNRAS, 427, 2349 
\bibitem{2019arXiv190505199C} Choksi, N., \& Gnedin, O.~Y.\ 2019, arXiv:1905.05199 
\bibitem{2012MNRAS.426..601C} Cole, D.~R., Dehnen, W., Read, J.~I., \& Wilkinson, M.~I.\ 2012, MNRAS, 426, 601 
\bibitem{2017ApJ...837...54C} Cole, A.~A., Weisz, D.~R., Skillman, E.~D., et al.\ 2017, ApJ, 837, 54 
\bibitem{2013ARA&A..51..393C} Conroy, C.\ 2013, ARA\&A, 51, 393
\bibitem{2001ApJ...559..828C} C{\^o}t{\'e}, P., McLaughlin, D.~E., Hanes, D.~A., et al.\ 2001, ApJ, 559, 828 
\bibitem{1998ApJ...501..554C} C{\^o}t{\'e}, P., Marzke, R.~O., \& West, M.~J.\ 1998, ApJ, 501, 554 
\bibitem{2009ApJ...695..101D} Damjanov, I., McCarthy, P.~J., Abraham, R.~G., et al.\ 2009, ApJ, 695, 101
\bibitem{2001ApJ...548L..33D} Davies, R.~L., Kuntschner, H., Emsellem, E., et al.\ 2001, ApJL, 548, L33 
\bibitem{1962ApJ...136..748E} Eggen, O.~J., Lynden-Bell, D., \& Sandage, A.~R.\ 1962, ApJ, 136, 748 
\bibitem{2019MNRAS.482.4528E} El-Badry, K., Quataert, E., Weisz, D.~R., Choksi, N., \& Boylan-Kolchin, M.\ 2019, MNRAS, 482, 4528 
\bibitem{1997ApJ...480..235E} Elmegreen, B.~G., \& Efremov, Y.~N.\ 1997, ApJ, 480, 235
\bibitem{2001ApJ...561..751F} Fall, S.~M., \& Zhang, Q.\ 2001, ApJ, 561, 751
\bibitem{}Ferreras, I NEED REFERENCE in press i think
\bibitem{}Forbes D.~A., et al., 2018, RSPSA, 474, 20170616
\bibitem{2018MNRAS.481.5592F} Forbes, D.~A., Read, J.~I., Gieles, M., \& Collins, M.~L.~M.\ 2018, MNRAS, 481, 5592 
\bibitem{}Forbes, D.~A.\ 2017, MNRAS, 472, L104 
\bibitem{1985ApJ...293..102F} Forman, W., Jones, C., \& Tucker, W.\ 1985,ApJ, 293, 102
\bibitem{1993ASPC...48..608F} Freeman, K.~C.\ 1993, The Globular Cluster-galaxy Connection, 608
\bibitem{1998ApJ...503..518F} Fukugita, M., Hogan, C.~J., \& Peebles, P.~J.~E.\ 1998, ApJ, 503, 518
\bibitem{2005MNRAS.362...41G} Gallazzi, A., Charlot, S., Brinchmann, J., White, S.~D.~M., \& Tremonti, C.~A.\ 2005, MNRAS, 362, 41 
\bibitem{1996AJ....111.1529G} Geisler, D., Lee, M.~G., \& Kim, E.\ 1996, AJ, 111, 1529
\bibitem{1997ApJ...474..223G} Gnedin, O.~Y., \& Ostriker, J.~P.\ 1997, ApJ, 474, 223
\bibitem{2019ApJ...876...39G} Gonz{\'a}lez-L{\'o}pezlira, R.~A., Mayya, Y.~D., Loinard, L., et al.\ 2019, ApJ, 876, 39 
\bibitem{}Gratton, R.~G., Carretta, E., \& Bragaglia, A. 2012, A\&ARv, 20, 50
\bibitem{1999AJ....118.1268G} Gibson, B.~K., Madgwick, D.~S., Jones, L.~A., et al.\ 1999, AJ, 118, 1268
\bibitem{2017ApJ...835..101H} Harris, W.~E., Ciccone, S.~M., Eadie, G.~M., et al.\ 2017, ApJ, 835, 101
\bibitem{1996AJ....112.1487H} Harris, W.~E.\ 1996, AJ, 112, 1487
\bibitem{}Harris W.~E., 1991, ARA\&A, 29, 543
\bibitem{1981AJ.....86.1627H} Harris, W.~E., \& van den Bergh, S.\ 1981, AJ, 86, 1627 
\bibitem{2014ApJ...787L...5H} Hudson, M.~J., Harris, G.~L., \& Harris, W.~E.\ 2014, ApJL, 787, L5 
\bibitem{2018MNRAS.477.3869H} Hudson, M.~J., \& Robison, B.\ 2018, MNRAS, 477, 3869 
\bibitem{2000AJ....119.1225H} Hughes, J., \& Wallerstein, G.\ 2000, AJ, 119, 1225
%\bibitem{2003gmbp.book.....H} Heggie, D., \& Hut, P.\ 2003, The Gravitational Million-Body Problem: A Multidisciplinary Approach to Star Cluster Dynamics, by Douglas Heggie and Piet Hut.~ Cambridge University Press, 2003, 372 pp.  
\bibitem{2006ApJ...646..899H} Humphrey, P.~J., Buote, D.~A., Gastaldello, F., et al.\ 2006, ApJ, 646, 899
\bibitem{2009ApJ...698.2048J} Johnson, C.~I., Pilachowski, C.~A., Michael Rich, R., et al.\ 2009, ApJ, 698, 2048
\bibitem{2007ApJS..171..101J} Jord{\'a}n, A., McLaughlin, D.~E., C{\^o}t{\'e}, P., et al.\ 2007, ApJS, 171, 101 
\bibitem{2014MNRAS.444.2377K} Katz, H., \& Ricotti, M.\ 2014, MNRAS, 444, 2377 
\bibitem{2014Natur.506..463K} Keller, S.~C., Bessell, M.~S., Frebel, A., et al.\ 2014, Nature, 506, 463 
\bibitem{1998ARA&A..36..189K} Kennicutt, R.~C.\ 1998, ARA\&A, 36, 189
\bibitem{2018MNRAS.474.4232K} Kim, J.-h., Ma, X., Grudi{\'c}, M.~Y., et al.\ 2018, MNRAS, 474, 4232 
\bibitem{1962AJ.....67..471K} King, I.\ 1962, AJ, 67, 471
\bibitem{2013ApJ...779..102K} Kirby, E.~N., Cohen, J.~G., Guhathakurta, P., et al.\ 2013, ApJ, 779, 102 
%\bibitem{2019ApJ...872..202K} Ko, Y., Lee, M.~G., Park, H.~S., et al.\ 2019, ApJ, 872, 202
\bibitem{2005ApJ...623..650K} Kravtsov, A.~V., \& Gnedin, O.~Y.\ 2005, ApJ, 623, 650  
\bibitem{2019MNRAS.486L..20K} Kruijssen, J.~M.~D.\ 2019, MNRAS, 486, L20 
\bibitem{2015MNRAS.454.1658K} Kruijssen, J.~M.~D.\ 2015, MNRAS, 454, 1658
\bibitem{2001AJ....121.2950K} Kundu, A., \& Whitmore, B.~C.\ 2001, AJ, 121, 2950
\bibitem{2013MNRAS.433.3017L} La Barbera, F., Ferreras, I., Vazdekis, A., et al.\ 2013, MNRAS, 433, 3017
\bibitem{2003ApJ...585..767L} Larsen, S.~S., Brodie, J.~P., Beasley, M.~A., et al.\ 2003, ApJ, 585, 767 
\bibitem{2013MNRAS.436..122L} Leaman, R., VandenBerg, D.~A., \& Mendel, J.~T.\ 2013, MNRAS, 436, 122
\bibitem{2019arXiv190611261M} Ma, X., Grudi{\'c}, M.~Y., Quataert, E., et al.\ 2019, arXiv:1906.11261 
\bibitem{2016MNRAS.460L.114M} Mackey, A.~D., Beasley, M.~A., \& Leaman, R.\ 2016, MNRAS, 460, L114
\bibitem{2019arXiv190508951M} Madau, P., Lupi, A., Diemand, J., et al.\ 2019, arXiv e-prints, arXiv:1905.08951
\bibitem{2018MNRAS.475.3700M} Mart{\'{\i}}n-Navarro, I., Vazdekis, A., Falc{\'o}n-Barroso, J., et al.\ 2018, MNRAS, 475, 3700 
\bibitem{2005MNRAS.361.1287M} Mandelbaum, R., Hirata, C.~M., Seljak, U., et al.\ 2005, MNRAS, 361, 1287
\bibitem{2018ApJ...861..148M} Mandelker, N., van Dokkum, P.~G., Brodie, J.~P., van den Bosch, F.~C., \& Ceverino, D.\ 2018, ApJ, 861, 148 
\bibitem{2005MNRAS.362..799M} Maraston, C.\ 2005, MNRAS, 362, 799
\bibitem{2009ApJ...694.1498M} Mar{\'\i}n-Franch, A., Aparicio, A., Piotto, G., et al.\ 2009, ApJ, 694, 1498
\bibitem{2011A&A...532A...8M} Marino, A.~F., Sneden, C., Kraft, R.~P., et al.\ 2011, AAP, 532, A8
\bibitem{2010A&A...519A..14M} Martell, S.~L., \& Grebel, E.~K.\ 2010, AAP, 519, A14
\bibitem{2019arXiv190608271M} Massari, D., Koppelman, H.~H., \& Helmi, A.\ 2019, arXiv e-prints, arXiv:1906.08271
\bibitem{2012AJ....144....4M} McConnachie, A.~W.\ 2012, AJ, 144, 4
\bibitem{2009Natur.461...66M} McConnachie, A.~W., Irwin, M.~J., Ibata, R.~A., et al.\ 2009, Nature, 461, 66 
\bibitem{1997A&ARv...8....1M} Meylan, G., \& Heggie, D.~C.\ 1997, A\&ARv, 8, 1
\bibitem{2015ads..book.....M} Michaud, G., Alecian, G., \& Richer, J.\ 2015, Atomic Diffusion in Stars, ISBN 978-3-319-19854-5
\bibitem{1996ApJ...461L..13M} Moore, B.\ 1996, ApJL, 461, L13
\bibitem{2017ARA&A..55...59N} Naab, T., \& Ostriker, J.~P.\ 2017, ARA\&A, 55, 59
\bibitem{2012MNRAS.421.1485N} Norris, M.~A., Gebhardt, K., Sharples, R.~M., et al.\ 2012, MNRAS, 421, 1485 
\bibitem{1995ApJ...447..680N} Norris, J.~E., \& Da Costa, G.~S.\ 1995, ApJ, 447, 680
\bibitem{2004AJ....127.2674O} Olsen, K.~A.~G., Miller, B.~W., Suntzeff, N.~B., Schommer, R.~A., \& Bright, J.\ 2004, AJ, 127, 2674 
\bibitem{1998MNRAS.300..665O} Olsen, K.~A.~G., Hodge, P.~W., Mateo, M., et al.\ 1998, MNRAS, 300, 665 
\bibitem{2019MNRAS.tmp.1624O} Orkney, M.~D.~A., Read, J.~I., Petts, J.~A., \& Gieles, M.\ 2019, MNRAS in press, arXiv:1906.04759
\bibitem{1984ApJ...277..470P} Peebles, P.~J.~E.\ 1984, ApJ, 277, 470
\bibitem{2011ApJ...730...23P} Peng, E.~W., Ferguson, H.~C., Goudfrooij, P., et al.\ 2011, ApJ, 730, 23
\bibitem{2006ApJ...639...95P} Peng, E.~W., Jord{\'a}n, A., C{\^o}t{\'e}, P., et al.\ 2006, ApJ, 639, 95
\bibitem{1987PASP...99...20P} Peterson, C.~J., \& Reed, B.~C.\ 1987, PASP, 99, 20
\bibitem{}Pfeffer, J., Kruijssen, J.~M.~D., Crain, R.~A., \& Bastian, N.\ 2018, MNRAS, 475, 4309 
%\bibitem{2003Msngr.114...53R} Renzini, A.\ 2003, The Messenger, 114, 53
\bibitem{2019MNRAS.484L..19P} Piatti, A.~E., Alfaro, E.~J., \& Cantat-Gaudin, T.\ 2019, MNRAS, 484, L19 
\bibitem{2013MNRAS.428..389P} Pota, V., Forbes, D.~A., Romanowsky, A.~J., et al.\ 2013, MNRAS, 428, 389 
\bibitem{2016ApJ...829L...5P} Powalka, M., Puzia, T.~H., Lan{\c c}on, A., et al.\ 2016, ApJL, 829, L5 
\bibitem{2019MNRAS.485.5861P} Pozzetti, L., Maraston, C., \& Renzini, A.\ 2019, MNRAS, 485, 5861
\bibitem{2002A&A...391..453P} Puzia, T.~H., Zepf, S.~E., Kissler-Patig, M., et al.\ 2002, AAP, 391, 453 
\bibitem{2017MNRAS.469L..63R} Renzini, A.\ 2017, MNRAS, 469, L63
\bibitem{2006ARA&A..44..141R} Renzini, A.\ 2006, ARA\&A, 44, 141
\bibitem{1970ApJ...159..379R} Rubin, V.~C., \& Ford, W.~K.\ 1970, ApJ, 159, 379
\bibitem{2009AJ....137.4956R} Romanowsky, A.~J., Strader, J., Spitler, L.~R., et al.\ 2009, AJ, 137, 4956 
\bibitem{2012MNRAS.424.2614S} S{\'a}nchez-Janssen, R., \& Aguerri, J.~A.~L.\ 2012, MNRAS, 424, 2614
\bibitem{2007ApJS..171..146S} Schiavon, R.~P.\ 2007, ApJS, 171, 146
\bibitem{2010A&A...513A..52S} Schuberth, Y., Richtler, T., Hilker, M., et al.\ 2010, AAP, 513, A52
\bibitem{1978ApJ...225..357S} Searle, L., \& Zinn, R.\ 1978, ApJ, 225, 357 
\bibitem{1995A&A...298..405S} Surma, P., \& Bender, R.\ 1995, AAP, 298, 405 
\bibitem{} Silk J., Di Cintio A., Dvorkin I., 2014, nhoc.conf,  137, nhoc.conf
\bibitem{} Simon, J. ARAA arXiv TO BE UPDATED
\bibitem{2015MNRAS.454.2502S} Smith, R., S{\'a}nchez-Janssen, R., Beasley, M.~A., et al.\ 2015, MNRAS, 454, 2502
\bibitem{2001ARA&A..39..137S} Sofue, Y., \& Rubin, V.\ 2001, ARA\&A, 39, 137
\bibitem{2011ApJS..197...33S} Strader, J., Romanowsky, A.~J., Brodie, J.~P., et al.\ 2011, ApJS, 197, 33
\bibitem{2007AJ....133.2015S} Strader, J., Beasley, M.~A., \& Brodie, J.~P.\ 2007, AJ, 133, 2015
\bibitem{2005AJ....130.1315S} Strader, J., Brodie, J.~P., Cenarro, A.~J., Beasley, M.~A., \& Forbes, D.~A.\ 2005, AJ, 130, 1315 
\bibitem{2019ApJ...871...58T} Tang, B., Liu, C., Fern{\'a}ndez-Trincado, J.~G., et al.\ 2019, ApJ, 871, 58
\bibitem{2000AJ....119.1645T} Trager, S.~C., Faber, S.~M., Worthey, G., et al.\ 2000, AJ, 119, 1645
\bibitem{2004ApJ...613..898T} Tremonti, C.~A., Heckman, T.~M., Kauffmann, G., et al.\ 2004, ApJ, 613, 898 
\bibitem{2014ApJ...780L..20T} Trujillo, I., Ferr{\'e}-Mateu, A., Balcells, M., Vazdekis, A., \& S{\'a}nchez-Bl{\'a}zquez, P.\ 2014, ApJL, 780, L20
\bibitem{2012MNRAS.426.1475U} Usher, C., Forbes, D.~A., Brodie, J.~P., et al.\ 2012, MNRAS, 426, 1475
\bibitem{2018Natur.555..629V} van Dokkum, P., Danieli, S., Cohen, Y., et al.\ 2018, Nature, 555, 629 
\bibitem{2015ApJ...798L..45V} van Dokkum, P.~G., Abraham, R., Merritt, A., et al.\ 2015, ApJL, 798, L45 
\bibitem{2013ApJ...775..134V} VandenBerg, D.~A., Brogaard, K., Leaman, R., et al.\ 2013, ApJ, 775, 134
\bibitem{2019MNRAS.483.3618V} Vanzella, E., Calura, F., Meneghetti, M., et al.\ 2019,MNRAS, 483, 3618
\bibitem{2017MNRAS.467.4304V} Vanzella, E., Calura, F., Meneghetti, M., et al.\ 2017, MNRAS, 467, 4304 
\bibitem{2019MNRAS.484.2832V} Vasiliev, E.\ 2019, MNRAS, 484, 2832
\bibitem{2001ApJ...549..274V} Vazdekis, A., Salaris, M., Arimoto, N., et al.\ 2001, ApJ, 549, 274
\bibitem{2010MNRAS.404.1639V} Vazdekis, A., S{\'a}nchez-Bl{\'a}zquez, P., Falc{\'o}n-Barroso, J., et al.\ 2010, MNRAS, 404, 1639
\bibitem{2019ApJ...873..118W} Watkins, L.~L., van der Marel, R.~P., Sohn, S.~T., et al.\ 2019, ApJ, 873, 118
\bibitem{2012AJ....144...76W} Willman, B., \& Strader, J.\ 2012, AJ, 144, 76
\bibitem{2006Sci...311.1129Y} Yoon, S.-J., Yi, S.~K., \& Lee, Y.-W.\ 2006, Science, 311, 1129 
\bibitem{2000AJ....120.2928Z} Zepf, S.~E., Beasley, M.~A., Bridges, T.~J., et al.\ 2000, AJ, 120, 2928 
\bibitem{1993MNRAS.264..611Z} Zepf, S.~E., \& Ashman, K.~M.\ 1993, MNRAS, 264, 611
\bibitem{2014ApJ...792...59Z} Zhu, L., Long, R.~J., Mao, S., et al.\ 2014, ApJ, 792, 59 
%
\end{thebibliography}

